Co-trading networks for modeling dynamic interdependency structures and estimating high-dimensional covariances in US equity markets

The time proximity of trades across stocks reveals interesting topological structures of the equity market in the United States. In this article, we investigate how such concurrent cross-stock trading behaviors, which we denote as co-trading, shape the market structures and affect stock price co-movements. By leveraging a co-trading-based pairwise similarity measure, we propose a novel method to construct dynamic networks of stocks. Our empirical studies employ high-frequency limit order book data from 2017-01-03 to 2019-12-09. By applying spectral clustering on co-trading networks, we uncover economically meaningful clusters of stocks. Beyond the static Global Industry Classification Standard (GICS) sectors, our data-driven clusters capture the time evolution of the dependency among stocks. Furthermore, we demonstrate statistically significant positive relations between low-latency co-trading and return covariance. With the aid of co-trading networks, we develop a robust estimator for high-dimensional covariance matrix, which yields superior economic value on portfolio allocation. The mean-variance portfolios based on our covariance estimates achieve both lower volatility and higher Sharpe ratios than standard benchmarks.

==> abstract_long.tex <==
The time proximity of trades across stocks reveals interesting topological structures of the equity market in the United States. In this article, we investigate how such concurrent cross-stock trading behaviors, which we denote as \textit{co-trading}, shape the market structures and affect stock price co-movements. By leveraging a co-trading-based pairwise similarity measure, we propose a novel method to construct dynamic networks of stocks. Our empirical studies employ high-frequency limit order book data from 2017-01-03 to 2019-12-09. By applying spectral clustering on co-trading networks, we uncover economically meaningful clusters of stocks. Beyond the static Global Industry Classification Standard (GICS) sectors, our data-driven clusters capture the time evolution of the dependency among stocks. Furthermore, our co-trading networks bridge the trading behaviors at a granular level with price co-movements among individual stocks. By conducting regression analysis, we demonstrate statistically significant positive relations between low-latency co-trading networks and realized covariance matrices of stocks returns. With the aid of co-trading networks, we develop a robust estimator for high-dimensional covariance matrices, which yields superior economic value on portfolio allocation. The mean-variance portfolios based on our covariance estimates generally outperform the baselines by achieving lower volatility and higher Sharpe ratios. Our best-performing portfolio achieves a Sharpe ratio of 1.40, which is 0.43 higher than the corresponding baseline, and 0.57 higher than the market over the same period.  



==> figure_list.tex <==
\newpage
 

\begin{figure}[t]
    \centering
    \includegraphics[width = \textwidth]{graphs/Co-occurrence_of_trades.pdf}
    \vspace{-4mm}  
    \caption{Illustration of trade co-occurrence. This figure visualizes the idea of co-occurrence of trades. With a pre-defined neighbourhood size $\delta$, trade $x_l$ arrives within the $\delta$-neighbourhood of trade $x_k$, and thus they co-occur. In contrast, trade $x_n$ locates outside $x_k$'s \gr{$\delta$-}neighbourhood, and thus the two trades do not co-occur. 
    \gr{Trade $ x_n$ co-occurs with $x_m$, and both} %Both 
trade $x_l$ and \gr{trade} $x_m$ co-occur with trade $x_k$, but they do not co-occur with each other. 
%Both trades $x_l$ and $x_m$ co-occur with trade $x_k$, but they do not co-occur with each other. 
}  
    \label{fig:trade_cooccurrence}
\end{figure}

\clearpage


\begin{figure}[t]
    \centering
    \includegraphics[width = 1\textwidth]{graphs/cooc_all_all_count_0.0005.pdf}
    \caption{\small A co-trading network of the period from 2017-01-03 to 2019-12-09. \\ The figure presents the co-trading network of 457 stocks represented by the co-trading matrix, without trading directions, of the entire period of study, that is $\mathbf{C}_{2017-2019}$. Each node represents a stock, whose color indicates its GICS sector. For visualization, we use \gr{a} maximum spanning tree (\cite{mantegna1999hierarchical}) to filter out edges by maximizing sum of co-trading scores while keeping a connected network with 456 edges.}  
    \label{fig:mst_cooc_network_plot}
\end{figure}

\clearpage



\begin{figure}[t]
    \centering
    \includegraphics[width = 1\textwidth]{graphs/sectorMetaGraph.pdf}
    \caption{\small Meta-flow network of GICS sectors. \\ This figure illustrates the fully connected network of GICS sectors based %upon 
    \gr{on the} co-trading matrix $C_{2017-2019}$. The edges are calculated by grouping stocks by their GICS sectors and averaging the co-trading scores of sector groups. }
    \label{fig:sector_meta_graph}
\end{figure}


\clearpage

\begin{figure}[t] % tp
    \centering
    \includegraphics[width = 1\textwidth]{graphs/all_all_count_0.0005_clusters.pdf}
    \caption{\small Clusters v.s. sectors. \\ This plot visualizes the overlap between the data-driven clusters, derived from $\mathbf{C}_{2017-2019}$ by spectral clustering, and the GICS sectors. The horizontal axis indexes stocks grouped by data-driven clusters, separated by vertical lines. The vertical axis indicates GICS sector labels. \mc{The colored area of a sector is indicative of its size.} } %The Financial stocks are well grouped in Cluster 1, while the Information Technology stocks are spread over multiple clusters, with a strong presence in Cluster 8.} }
    \label{fig:cooc_clusters_plot}
\end{figure}



\clearpage

\begin{figure}[t]
    \begin{subfigure}{\textwidth}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/circle_cooc_net_0.0005_all_all_201701.pdf}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/circle_cooc_net_0.0005_all_all_201801.pdf}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]
    {graphs/circle_cooc_net_0.0005_all_all_201901.pdf}
    \end{subfigure}
    \end{subfigure}

    \iffalse
    \begin{subfigure}{\textwidth}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/heatmap_cooc_mat_2017-01.pdf}
    \caption{\small 2017-01}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/heatmap_cooc_mat_2018-01.pdf}
    \caption{\small 2018-01}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]
    {graphs/heatmap_cooc_mat_2019-01.pdf}
    \caption{\small 2019-01}
    \end{subfigure}
    \end{subfigure}
    \fi
    
    \begin{subfigure}{\textwidth}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/heatmap_cooc_mat_2017-01_yl.pdf}
    \caption{\small 2017-01}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]{graphs/heatmap_cooc_mat_2018-01_yl.pdf}
    \caption{\small 2018-01}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width = \textwidth, height = \textwidth]
    {graphs/heatmap_cooc_mat_2019-01_yl.pdf}
    \caption{\small 2019-01}
    \end{subfigure}
    \end{subfigure}


    \caption{\small Thresholded temporal co-trading networks. \\ These three networks are based on co-occurrence of all trades regardless of trading directions. For visualization, we threshold on co-trading scores and only keep top $1 \%$ of edges. The first row contains the thresholded networks and the second row includes heatmaps of the corresponding co-trading matrices. From left to right, are networks and co-trading matrices of 2017-01, 2018-01 and 2019-01. Colors stand for the GICS sectors. } \label{fig:threshold_cooc_net} 
\end{figure}


\clearpage


\begin{figure}[t]
    \centering
    \includegraphics[width = \textwidth]{graphs/sectorClusterARI.pdf}
    \caption{\small Adjusted Rand index between daily clusters and GICS sectors. \\ This figure sketches dynamics similarity between data-driven clusters and GICS sectors. \gr{For e}very day, we derive data-driven clusters and calculate the adjusted Rand index with GICS, with predefined numbers of clusters  $\{11, 15, 20, 50\}$. We then plot the ARIs over time from 2017-01-03 to 2019-12-09, %and
    \gr{so that} each line represents one \gr{choice} %value 
    of \gr{number of} clusters. %numbers.
    }
    \label{fig:sector_cluster_ari}
\end{figure}



\clearpage



\begin{figure}[h]
    \centering
    \includegraphics[width = 0.5\textwidth]{graphs/temporalClustersHeatmapAllC20.png}
    \caption{\small Similarity of daily clusters. \\ This heatmap shows the similarity between days. Every day, we group stocks into 20 clusters by applying spectral clustering on the daily co-trading matrix. Then, for each pair of days, we calculate \gr{the} ARI between the clusters. }
    \label{fig:temporal_ari_heatmap}
\end{figure}



\clearpage



\begin{figure}[h]
    \centering
    \includegraphics[width = 1\textwidth]{graphs/temporalClustersAllC20.pdf}
    \caption{\small Regimes detected by spectral clustering. \\ This figure shows the clusters of days, derived by applying spectral clustering on the heatmap of ARI in Figure \ref{fig:temporal_ari_heatmap} to classify days into three regimes. The horizontal axis indicates dates and the vertical axis indicates which cluster each day belongs to.}
    \label{fig:temporal_clusters_plot}
\end{figure}


\clearpage




\begin{figure}[h]
    \centering
    \includegraphics[width = \textwidth]{graphs/mvVolatilityLeverage.pdf}
    \vspace{-4mm}  
    \caption{Annualized volatility of mean-variance portfolios. \\ These figures show the annualized volatility of mean-variance portfolios constructed by solving \eqref{eq:mv_opt} based on different covariance matrices estimates. The out-of-sample backtests span the period from 2017-01-03 to 2019-12-09. Every sub-figure corresponds to one choice of latent factor numbers while decomposing sample covariance matrices in \eqref{eq:decompose_covariance}.
    %\GR{explain how: according to ... ?}
    In each sub-figure, every curve plots portfolio volatility, for a choice of blocks structure imposed on the residual covariance, along leverage constraints.} 
    \label{fig:mv_volatility}
\end{figure} 

\clearpage


\begin{figure}[t]
    \centering
    \includegraphics[width = \textwidth]{graphs/mvBenchmarkPnl.pdf}
    \vspace{-4mm}  
    \caption{Cumulative returns of portfolios. \\ This figure plots cumulative returns of four portfolios from 2017-01-03 to 2019-12-09. The portfolios include (1) `GMV-cluster': the global minimum variance portfolio based on robust covariance matrices estimated using our method with 10 factors and 20 clusters; (2) `GMV-cluster': the GMV portfolio based on robust covariance matrices estimated using 10 factors and GICS sectors; (3) `SPY (close to close)': the SPDR S$\&$P 500 ETF Trust which tracks the S$\&$P 500 Index; (4) `SPY (open to close)': the SPY ETF, following our strategy, with positions only during normal trading hours.} 
    \label{fig:mv_benchmark_pnl}
\end{figure}


\clearpage


\begin{figure}[htp]
    \centering
    \includegraphics[width = \textwidth]{graphs/clusterRobustARI.pdf}
    \vspace{-4mm}  
    \caption{Robustness of applying spectral clustering on daily co-trading networks. \\ This figure plots the daily means of ARIs between each pair of clusters obtained by running the spectral clustering method 100 times on the same co-trading matrix every day, with different random initialization. Each line corresponds to a value of number of clusters, chosen from 11, 15, 20 and 50.} 
    \label{fig:clustering_robustness}
\end{figure}



==> input_main.tex <==



We investigate concurrent (almost instantaneous) trading across multiple stocks, a phenomenon which we refer to as \textit{co-trading} behavior, at a very granular level by directly considering individual trades, and zooming-in around their local neighborhoods. 

In this paper, we propose a novel method that constructs \textit{co-trading networks}, in order to model the complex structures of co-trading activities in equity markets. Constructed from limit order books, our co-trading networks bridge the trading behaviors at a granular level with the dynamic topological structures of the equity market and price co-movements among individual stocks. Moreover, by making use of co-trading networks, we develop a robust estimator for high-dimensional covariance matrices, and demonstrate  its conspicuous economic value on portfolio allocation. 
 
The network construction starts with a pairwise similarity measure between stocks. Inspired by the idea of trade co-occurrence originating from \cite{lu2022trade}, we define the pairwise similarity as the normalized count of times that trades, for a given pair of stocks, arrive concurrently. We name this measure as a \textit{co-trading score}, since it embeds the intuition that stocks frequently traded together are closely related. Concatenating co-trading scores between every pair of stocks, we obtain the co-trading matrix, which serves as the adjacency matrix of the proposed weighted network of equity markets. 

Utilizing algorithms and tools for network analysis (\cite{hagberg2008exploring}), we provide empirical evidence that co-trading networks are capable of capturing meaningful structures of the equity market. By visualizing a co-trading network, aggregated over the entire period of study, with information filtering (\cite{mantegna1999hierarchical}), we observe that stocks from the same sector groups tend to have strong co-trading relations. This observation echos the phenomenon that often stocks in the same sector groups of the market are likely to appear in the same portfolios and their prices tend to move together. Additionally, we uncover clusters, or communities, of stocks in the co-trading network. To detect these communities, we apply a spectral clustering algorithm on the co-trading matrix to group stocks with similar co-trading behaviors into clusters. For comparison, we select the Global Industry Classification Standard (GICS) as sector labels. Our empirical results show substantial overlap between the data-driven clusters and GICS sectors, which confirms that the co-trading network accommodate the sector structures as expected. Moreover, we leverage the uncovered network to study the influence of both individual stocks and sectors on the market. By using tools such as  eigenvector centrality (\cite{bonacich1972factoring}, \cite{bonacich1987power}), we identify that large technology companies and financial institutions, such as Microsoft, Apple, and JPMorgan, present stronger co-trading relations with others, thus have higher impact on the structure of the market. Despite the alignment with GICS sectors, the co-trading network also contains information beyond sectorial structure. The data-driven clusters also group together closely related stocks from different sectors. 

Apart from the aforementioned static graph, the construction of co-trading matrices is flexible due to the choice of distance in time at which two trades are deemed to co-occur. It is also informative to analyze the time evaluation of co-trading networks and explore the dynamic of market structures. In this study, we focus on network time series at daily level, but this approach can be easily be generalized to intraday, monthly and so forth. Our empirical findings from daily co-trading networks indicates that the co-trading relations across different sectors increase from 2017 to 2019. Using spectral clustering, we detect clusters at a daily level and compare them with GICS sectors. By plotting the similarity across time, we observe a downward trend with fluctuations. In addition, we also compare the similarity among daily clusters. The variation in clusters also increases as the spread of co-trading beyond sector groups. By applying the spectral clustering algorithm for change-point detection based on the temporal similarity heatmap, we uncover three distinct regimes over the period of study.

To exploit the association between co-trading behaviors and price co-movements, we conduct network regression analysis. We build realized covariance matrices from intraday returns as proxies for co-movements among stocks. By regressing covariance matrices against co-trading networks on a daily basis, we reveal  positive associations between the two types of matrices. Furthermore, on $98.51 \%$ of the days in the study, the positive regression coefficients are statistically significant at $5 \%$ significance level. Further controlling for GICS sectors, we conduct multiple regressions by adding a fixed sector network as an independent variable. Even with the presence of sectors, the positive and significant relation still holds. Therefore, there is a strong indication that the co-trading behaviors at the high-frequency level are positively correlated with the return covariance, and have explainability power on price co-movements that goes beyond the  commonly adopted sectors. 

With the aid of co-trading matrices, we propose a robust estimator for the high-dimensional covariance matrix of stock returns at daily frequency. By assuming that  stock returns follow a linear factor structure (\cite{ross1976arbitrage}), we  decompose the  covariance matrix as the sum of the factor covariance and the idiosyncratic covariance. Then, we impose a block structure on the diagonal of the idiosyncratic covariance matrix, such that elements outside the blocks are set to zero. Our approach extends the work of \cite{ait2017using}, which use principle component analysis to derive latent factors and form blocks using GICS sectors. However, as the GICS sectors are fixed, the sector blocks remain static over time. As we have shown,   the market structures are time-varying, and thus static sector memberships  are not enough to capture the similarity of stocks at higher frequency. Therefore, we update the diagonal block structure daily with data-driven clusters derived from co-trading networks. To evaluate the performance, we construct mean-variance portfolios, subject to various leverage constraints. Our covariance estimators, based on dynamic clusters, generally outperform the baselines, using fixed GICS sectors, by achieving lower volatility and higher Sharpe ratios. Our best-performing portfolio achieves a Sharpe ratio of 1.40, which is 0.43 higher than the corresponding baseline, and 0.57 higher than the market over the same period.  

==> table_list.tex <==
\newpage

\begin{table}[h]
    \caption{Top 10 stocks by eigenvector centrality. \\ This table lists 10 stocks ranked by their eigenvector centrality, as well as their company names and GICS sectors.}    
    \input{tables/topCetralityComp.tex}
    \label{tab:top_centrality_comp}
\end{table}


\newpage

\begin{table}[h]
    \caption{Centrality of sectors in \gr{the} meta-flow network. \\ This table shows the eigenvector centrality of each GICS sector in the meta-flow network. The `Rank' column reports the rank, in descending order, of each sector in terms of their centrality.}    
    \input{tables/sectorMetaCentrality.tex}
    \label{tab:sector_meta_centrality}
\end{table}

\newpage

\begin{table}[h]
    \caption{Statistics of daily ARI. \\ This table shows summary statistics of daily ARIs between dynamic clusters and fixed GICS sectors plotted in Figure \ref{fig:sector_cluster_ari}. For different number of clusters, the table reports the mean and standard deviation of ARIs from 2017-01-03 to 2019-12-09, \gr{as well as the signal-to-noise ratio}.}    
    \input{tables/statsARI.tex}
    \label{tab:stats_ari}
\end{table}  


\newpage

\begin{table}[h]
    \caption{Simple network regression. \\ This table reports the mean, median and standard deviation of daily network regression coefficients in \eqref{reg_qap}, as well as their $p$-values. \gr{The $p$-values are obtained using the QAP with 2000 simulations.} We run one regression for each trading day from 2017-01-03 to 2019-12-09. %For inference, we use QAP and simulate 2000 times to calculate $p$-values.
    }    
    \input{tables/qap.tex}
    \label{tab:qap}
\end{table}

\newpage
\begin{table}[h]
    \caption{Multiple network regression. \\ This table reports the mean, median and standard deviation of daily network regression coefficients in \eqref{reg_mrqap}, as well as their $p$-values. We perform one regression for each trading day from 2017-01-03 to 2019-12-09. For inference, we use MRQAP with SDP, \mc{in line with \cite{dekker2007sensitivity}}  and simulate 2000 runs to calculate $p$-values.}    
    \input{tables/mrqap.tex}
    \label{tab:mrqap}
\end{table}


\newpage
\begin{table}[h]
    \caption{Annualized Sharpe ratio of mean-variance portfolios. \\ This table documents the annualized Sharpe ratios of mean-variance portfolios constructed by solving \eqref{eq:mv_opt} based on different covariance matrices estimates. The out-of-sample backtests span the period from 2017-01-03 to 2019-12-09. \gr{The} `Factor' column specifies the number of latent factors while decomposing the sample covariance matrices.  The `Leverage' column indicates leverage constraints in \eqref{eq:mv_opt}, where $\infty$ means that short-sell is unrestricted. We use 15, 20 and 50 clusters, together with GICS sectors as the baseline, while imposing \mc{diagonal block structure} on the residual covariance matrices.} 
    \input{tables/mvAnnualSharpe.tex}
    \label{tab:mv_sharpe}
\end{table}


\newpage
\begin{table}[htp]
    \caption{Summary of analysis on volume based co-trading matrices. \\ We construct volume based daily co-trading matrices from 2017-01-03 to 2019-12-09. Panel A reports the annualized Sharpe ratios of global minimum variance (GMV) portfolios constructed by solving \eqref{eq:mv_opt} based on different covariance matrices estimates. \gr{The} `Factor' column specifies the number of latent factors while decomposing the sample covariance matrices.  The `GICS' and `Count-20' columns indicate GMV portfolios corresponding to GICS and clustering count based co-trading matrices with 20 clusters as benchmarks. For volume based co-trading matrices, we use 15, 20 and 50 clusters while imposing \mc{diagonal block structure} on the residual covariance matrices. Additionally, we detect clusters of stocks on volume based co-trading matrices every day with 100 different random seeds for spectral clustering. The predefined number of clusters are 11, 15, 20 and 50. For comparison purpose, we report the statistics for clusters of count based co-trading matrices under. Each value in Panel B is a mean of ARIs between each pair of clusters every day and averaged over all days. Each value in Panel C represents a mean of ARIs between data-driven clusters and GICS sectors each day and averaged over all days.}    
    \input{tables/robustVolume.tex}
    \label{tab:robust_volume}
\end{table}

\clearpage




==> tables/marqap_backup.tex <==
\begin{tabularx}{\textwidth}{l*{5}{Y}}
\toprule
     & $\gamma_{t}^{C}$ & $p$-value  & $\gamma_{t}^{S}$ & $p$-value \\
\midrule
Mean &    3.61          &     0.030     &  0.24        &  0.001  \\
Median &    3.04        &     0.001     &  0.20        &   0.000  \\
Standard deviation &    2.52          &    0.116      &  0.16        &   0.009\\
Percentage positive &   99.73     & -   &  99.86    & - \\    
Percentage significant &    89.81 & -   &  99.56    & -\\
\bottomrule
\end{tabularx}
